Streaming Small-Footprint Keyword Spotting using Sequence-to-Sequence Models

We develop streaming keyword spotting systems using a recurrent neural network transducer (RNN-T) model: an all-neural, end-to-end trained, sequence-to-sequence model which jointly learns acoustic and language model components. Our models are trained to predict either phonemes or graphemes as subword units, thus allowing us to detect arbitrary keyword phrases, without any out-of-vocabulary words. In order to adapt the models to the requirements of keyword spotting, we propose a novel technique which biases the RNN-T system towards a specific keyword of interest. Our systems are compared against a strong sequence-trained, connectionist temporal classification (CTC) based "keyword-filler" baseline, which is augmented with a separate phoneme language model. Overall, our RNN-T system with the proposed biasing technique significantly improves performance over the baseline system.

==> _ <==
\section{Experimental Details}
\label{sec:experiments}

\subsection{Data and Evaluation Metric}

Our models are trained on a set of $\sim$22M hand-transcribed anonymized
utterances extracted from Google voice-search traffic, which corresponds to
$\sim$18,000 hours of training data.
In order to improve system robustness to noise and reverberation,
multi-condition training (MTR) data are generated: training utterances are
artificially distorted using a room simulator, by adding in noise samples
extracted from YouTube videos and environmental recordings of daily events.
To further improve robustness to variation in signal loudness, we perform
multi-loudness training by scaling the loudness of each training utterance to a
randomly selected level.
%ranging from −65 dBFS to −7 dBFS
%The overall SNR is between 0dB and 30dB, with an average of 12dB.

We construct separate development and test sets to measure KWS
performance.
As keyword phrases we consider personal names which contain three or more
syllables (e.g., \texttt{Olivia} or \texttt{Erica}).
The development set consists of 328 keywords, each of which is contained in
$\sim$75 positive utterances, collected from multiple speakers, of the form ``keyword, query'', (e.g.,
\texttt{Olivia, how tall is the Eiffel tower?}).
A set of $\sim$37K negative utterances ($\sim$50 hours in total) are shared
across keywords, which are collected as queries without a keyword, to form the
full development set.
Each keyword is evaluated separately on a set consisting of its own positive
utterances and the shared negative utterances.
A test set is created similarly, with 228 keywords each contained in $\sim$500
positive utterances, and a set of $\sim$20k negative utterances ($\sim$60
hours in total) shared across keywords, which consist of hand-transcribed
anonymized utterances extracted from Google traffic from the domains of
open-ended dictation and voice-search queries.

We evaluate performance in terms of the receiver operating characteristic (ROC)
curve~\cite{MohriCortes04}, which is constructed by sweeping a threshold over
all possible confidence values and plotting false reject (FR) rates against
false alarm (FA) rates. Our goal is to achieve low FR rates while maintaining
extremely low FA rates (e.g. no more than 0.1 false alarms per hour of audio).

Following~\cite{ZhangEtAl12}, we employ a score normalization approach to map
system confidence at the utterance level for a keyword to the probability of
false alarm (pFA) for that keyword, which allows us to use a single consistent
score for all keywords and set the decision threshold reliably.
A confidence to pFA rate mapping is estimated from the development set, and
applied to both the development and the test sets.
All ROC curve results in this work are plotted after the score normalization.

\subsection{Model Details}

The input acoustic signal is represented with 80-dimensional log-mel filterbank
energies, computed with a 25ms window, and a 10ms frame-shift.
Following previous work~\cite{SakSeniorRaoEtAl15}, we stack three consecutive
frames and present only every third stacked frame as input to the encoder.
The same acoustic frontend is used for all experiments described in this work.

The CTC acoustic model (AM) consists of 5 layers of 500 long short-term memory
(LSTM)~\cite{HochreiterSchmidhuber97} cells, that predict context-independent
phonemes as output targets.
The system is heavily compressed, both by
quantization~\cite{AlvarezPrabhavalkarBakhtin16}, and by the application of
low-rank projection layers with 200 units between consecutive LSTM
layers~\cite{PrabhavalkarAlsharifBruguierMcGraw17}.
The AM consists of 4.6 million parameters in total.
The model is first trained to optimize the CTC objective
function~\cite{GravesFernandezGomezEtAl06} until convergence.
Once CTC-training is complete, the model is discriminatively sequence-trained to
optimize expected word errors by minimizing word-level, edit-based, minimum Bayes
risk (EMBR) proposed recently by Shannon~\cite{Shannon17}.

The encoder networks used in all RNN transducer models are identical in size and
configuration to the CTC model.
During the training of an RNN transducer, the weights from the encoders are
initialized from a pre-trained CTC model, since this was found to significantly
speed up convergence, following which the weights are trained jointly with the
rest of the network.
For the RNN-T model that is trained to directly output grapheme targets, the CTC
model used for initialization is also trained to predict graphemes.
The grapheme inventory includes the 26 lower-case letters
(\texttt{a--z}), the numerals (\texttt{$0$--$9$}), a label representing `space'
(\texttt{$\spc$}), and punctuation
symbols (e.g., the apostrophe symbol (\texttt{'}), hyphen (\texttt{-}), etc.).

The prediction network used in the RNN transducer models, both with and without
attention, consists of a single layer of 500 LSTM cells with coupled input and
forget gates (CIFG)~\cite{ChoMerrienboerGulcehreEtAl14}, and the joint network
consists of a single feed-forward layer of 500 units with a $\tanh$ activation
function, as described in Section~\ref{sec:rnnt}.
The decoder network (including prediction network and the joint network) has 1.5
million parameters in total.

The RNN transducer models are decoded using a beam-search
algorithm~\cite{Graves12}, where at most 50 highest scoring candidates are
retained at every step during decoding.
In general, the output posterior distribution of sequence-to-sequence models
like RNN-T is peaky (i.e., low entropy); such over-confidence is typically
suboptimal to keyword spotting, since diversity in hypotheses is critical to
reduce the number of false rejects.
We find that smoothing the posteriors with a temperature $\tau$, i.e. dividing
the logits of the output layer by $\tau$ before softmax normalization, can help
improve KWS performance significantly.
The optimal temperature value is determined by tuning on the development set; we
set $\tau=2.0$ for all RNN-T models without attention, and $\tau=2.2$ for the
ones with attention.

The language model (LM) used in the keyword-filler model with CTC is trained to
predict phoneme targets on the same $\sim$22M utterances used for training RNN-T
models.
The LM is pruned to $\sim$1.5-million 6-grams using entropy pruning, similar to
the number of parameters in the decoder of our RNN-T models.
We choose $n=6$ which is optimized from the development set.

The LM for our embedded LVCSR system is a standard word-level 5-gram, which
is trained on a larger corpus with $\sim$100M automatically-transcribed
anonymized utterances extracted from Google voice-search traffic.
This LM is also pruned to $\sim$1.5-million n-grams using entropy pruning.
The vocabulary is limited to 64K words, allowing us to shrink the data
structures used to maintain the LM~\cite{McGrawPrabhavalkarAlvarezEtAl16}.
Note that the fixed vocabulary results in out-of-vocabulary keywords on the
development and test sets.
Utterances are decoded with a heavily pruned version of the LM in the
first-pass, while rescoring with the full LM on-the-fly, thus allowing us to
reduce the size of the decoder graph used in the first-pass.

All models are trained using asynchronous stochastic gradient
descent~\cite{DeanCorradoMongaEtAl12}, and are implemented in
TensorFlow~\cite{AbadiAgarwalBarhamEtAl15}.

